The Syncline Model -- Analyzing the Impact of Time Synchronization in Sensor Fusion

The accuracy of sensor fusion algorithms are limited by either the intrinsic sensor noise, or by the quality of time synchronization of the sensors. While the intrinsic sensor noise only depends on the respective sensors, the error induced by quality of, or lack of, synchronization depends on the dynamics of the vehicles and robotic system and the magnitude of time synchronization errors. To meet their sensor fusion requirements, system designers must consider both which sensor to use and also how to synchronize them. This paper presents the Syncline model, a simple visual model of how time synchronization affects the accuracy of sensor fusion for different mobile robot platform. The model can serve as a simple tool to determine which synchronization mechanisms should be used.

==> 7_future.tex <==
\section{Future Works}
The accuracy of the Syncline model is measured by simulating robot systems based on the same mathematical model which the Syncline model was derived from.
Evaluating the model on real, experimental data is left as future work.

==> app_equations.tex <==
\clearpage
\appendix
\section{System equations}
\begin{table}[h]
    \centering
    \caption{\label{tab:my_label}Caption}
    \begin{tabular}{cc}
    \toprule
    Symbol & Frame  \\ \midrule
     $\{e\}$     & ECEF  \\
     $\{n\}$     & NED  \\
     $\{g\}$     & GNSS location  \\
     $\{b\}$     & Body frame \\
     $\{u\}$     & USBL  \\
     $\{m\}$     & Multibeam location  \\
     $\{o\}$     & Object seen by multibeam \\
     \bottomrule
    \end{tabular}
\end{table}

\begin{equation}
    \begin{split}
    \bm p^e_{eo} &= 
    \underbrace{
    \bm p^e_{eg_\mathrm{sv}} + \bm 
    R_{en_\mathrm{sv}}\bm R_{n_\mathrm{sv}b_\mathrm{sv}} 
    \left(
    \bm p^{b_\mathrm{sv}}_{g_\mathrm{sv}u_\mathrm{sv}}
    + \bm p^{b_\mathrm{sv}}_{u_\mathrm{sv}u_\mathrm{auv}}\right)}_{\bm p^e_{eu_\mathrm{auv}}} \\ 
    & \quad +
    \underbrace{
    \bm R_{en_\mathrm{auv}}\bm R_{n_\mathrm{auv}b_\mathrm{auv}} 
    \left( 
    \bm p^{b_\mathrm{auv}}_{u_\mathrm{auv} m_\mathrm{auv}}
    +
    \bm p^{b_\mathrm{auv}}_{m_\mathrm{auv} o}
    \right)}_{\bm p^e_{u_\mathrm{uav}o}}
\end{split}
\end{equation}

Derivative of this is
\begin{equation}
    \begin{split}
    \bm v^e_{eo} &= 
    \bm v^e_{eg_\mathrm{sv}}\\ 
    &\quad + 
    \bm R_{en_\mathrm{sv}}
    \bm S(\bm \omega^{n_\mathrm{sv}}_{en_\mathrm{sv}})
    \bm R_{n_\mathrm{sv}b_\mathrm{sv}} 
    \left(
    \bm p^{b_\mathrm{sv}}_{g_\mathrm{sv}u_\mathrm{sv}}
    + \bm p^{b_\mathrm{sv}}_{u_\mathrm{sv}u_\mathrm{auv}}\right) \\
    & \quad +
    \bm R_{en_\mathrm{sv}}
    \bm R_{n_\mathrm{sv}b_\mathrm{sv}} 
    \bm S(\bm\omega^{b_\mathrm{sv}}_{n_\mathrm{sv}b_\mathrm{sv}})
    \left(
    \bm p^{b_\mathrm{sv}}_{g_\mathrm{sv}u_\mathrm{sv}}
    + \bm p^{b_\mathrm{sv}}_{u_\mathrm{sv}u_\mathrm{auv}}\right)
    \\
    &\quad+ 
    \bm R_{en_\mathrm{sv}}
    \bm R_{n_\mathrm{sv}b_\mathrm{sv}} 
    \bm v^{b_\mathrm{sv}}_{u_\mathrm{sv}u_\mathrm{auv}}
    \\ 
    &\quad + 
    \bm R_{en_\mathrm{auv}}
    \bm S(\bm\omega^{n_\mathrm{auv}}_{en_\mathrm{auv}})
    \bm R_{n_\mathrm{auv}b_\mathrm{auv}} 
    \left( 
    \bm p^{b_\mathrm{auv}}_{u_\mathrm{auv} m_\mathrm{auv}}
    +
    \bm p^{b_\mathrm{auv}}_{m_\mathrm{auv} o}
    \right)
    \\
    &\quad + 
    \bm R_{en_\mathrm{auv}}
    \bm R_{n_\mathrm{auv}b_\mathrm{auv}} 
    \bm S(\bm \omega^{b_\mathrm{auv}}_{n_\mathrm{auv}b_\mathrm{auv}})
    \left( 
    \bm p^{b_\mathrm{auv}}_{u_\mathrm{auv} m_\mathrm{auv}}
    +
    \bm p^{b_\mathrm{auv}}_{m_\mathrm{auv} o}
    \right)
\end{split}
\end{equation}
where
\begin{itemize}
    \item $\bm u^{b_\mathrm{sv}}_{b_\mathrm{sv}b_\mathrm{sv}}$ is the relative velocity of the AUV's USBL and the SV's USBL.
    \item $\bm \omega^{n_\mathrm{sv}}_{en_\mathrm{sv}}$ is the angular velocity of latitude and longitude / change in the horizontal position
\end{itemize}
\clearpage


==> dump.tex <==

\iffalse
That is, the rate of change of the internal state variables of the robot. 
We are interested in the worst case behaviour and define the vect
\begin{align}
  \bm{D_{max}} = \bm{max}(\frac{\Delta\bm{X}^{int}}{\Delta k})    
\end{align}
$\bm{D_{max}}$ is the maximum expected change to occur for the internal state variables in a clock period. This vector can be estimated with simulations or reasoning about the normal operation of the robot.
\fi


\iffalse
We simplify the LiDAR measurement to producing a range $r$ and a bearing $\bm{b} = [\phi, \theta]$. I.e. azimuth and elevation.
Range is simply the length of the vector between the CO of the LiDAR  and the object.

\begin{align}
    r &= |\bm{p}_{s/e}^e - \bm{p}_{s/e}^e| \\
\end{align}



To find the bearing we start with a unit vector in the ECEF frame from the CO of the robot to the object. And rotate twice

\begin{align}
    \bm{\lambda}_{e} &= \frac{\bm{p}_{o/e}^e - \bm{p}_{b/e}^e}{r} \\
    \bm{\lambda}_{s} &= \bm{R}_e^s\bm{R}_e^b\bm{\lambda}_e
\end{align}

We then see that the unit vector from the LiDAR to the object, $\bm{\lambda}_{s}$

\begin{align}
\bm{\lambda}_{s} = \begin{bmatrix}\cos\phi\cos\theta \\ \sin\phi\cos\theta \\ -\sin\phi \end{bmatrix}
\end{align}


where $\phi$ is the azimuth and $\theta$ is the elevation. We further see that
\begin{align}
    \phi &= \arctan\frac{\lambda_2}{\lambda_1} \\
    \theta &=\arctan\frac{\lambda_3}{\lambda_2}
\end{align}



So, to summarize our sensor sampling model is as follows:
\begin{equation}
  \bm{Y} =\begin{bmatrix}
  \bm{Y}^{INS} \\
  \bm{Y}^{LiDAR} \\
\end{bmatrix} = \begin{bmatrix}
\hat{\bm{p}}_{b/e}^e \\ \hat{\bm{\Theta}_{nb}} \\ \hat{r} \\ \hat{\phi} \\ \hat{\theta}
\end{bmatrix}
  \label{eq:sensor_sample_full}
\end{equation}


Here the hat indicate that we ar

\fi



\iffalse

We observe that the attitude error of the INS and the bearing error of the LiDAR affects the system in a similar way and are scaled by the range measurement. 
The position error is then added. Clearly the effects of sync noise depends on the numerical value of the range.
The expected range for georeferencing is a parameter to the syncbound model together with the expected dynamics of the system.




Now, our goal is to understand the causes of estimation error. We define the estimation error as:
\begin{align}
  \mathbf{e} &=  \mathbf{\hat{p}}_{o} - \mathbf{p}_{o} \\
  \mathbf{e} &= \bm{p}_{b/e}^e + r\bm{R}_b^e\bm{R}_{s}^b\bm{b}_{so}^{s} - (\bm{\hat{p}}_{b/e}^e + \hat{r}\bm{\hat{R}}_b^e\bm{R}_{s}^b\bm{\hat{b}}_{so}^{s})\\
  \mathbf{e} &= \bm{p}_{b/e}^e - \bm{\hat{p}}_{b/e}^e  + r\bm{R}_b^e\bm{R}_{s}^b\bm{b}_{so}^{s} - \hat{r}\bm{\hat{R}}_b^e\bm{R}_{s}^b\bm{\hat{b}}_{so}^{s} \\
\end{align}


First we simplify the rotation matrix from Body to NED which is the output from the INS. We can safely ignore the rotation from body to sensor because it is linear transformation.

\begin{equation}
\bm{R_{b}^{e}} = 
    \begin{bmatrix}
      1 & -\Psi & \theta \\
      \psi & 1 & - \phi \\
      -\theta & \phi & 1 \\
    \end{bmatrix}
\end{equation}

We then look at the x-component of the second part of the estimation error equation

\begin{align}
  r(b_{1}- \psi b_{2} + \theta b_{r}) - \hat{r}(\hat{b}_{1} - \hat{\psi}\hat{b_{2}} + \hat{\theta}\hat{b_{3}})
\end{align}




Our goal is to investigate the error which has two potential source.
Either white noise associated with the sensor or the synchronization noise introduced by synchronization precision.
We 

\fi


\iffalse
- SBG Ellipse: https://www.sbg-systems.com/wp-content/uploads/Ellipse_Series_Leaflet.pdf
- 0.05deg +/- RTK or 0.1deg SP Roll/Pitch
- 0.2deg heading dual antenna
- Navigation: 1m SBAS and 1cm RTK


- OUster OS1: https://data.ouster.io/downloads/datasheets/datasheet-revd-v2p1-os1.pdf
- 0.3m-1m: 0.7cm
- 1-20m: 1cm
- 20-50m: 2cm
- >50m: 5cm
- Range Accuracy: +/- 3cm or +/-10cm

- Q: What is it that the LiDAR is measuring? A: Range (dist) and Bearing (angle) to a bunch of points. Imagine that we are doing a 3D mapping.
\fi


==> thesis_include.tex <==
\input{0_abstract}
\newpage
\input{1_introduction}
\input{2_background}
\input{3_preliminaries}
\input{3_related}
\input{4_syncline}
\input{5_examples}
%\input{7_future}
\input{6_conclusion}

